Mixed Policy Gradient: off-policy reinforcement learning driven jointly by data and model

Reinforcement learning (RL) shows great potential in sequential decision-making. At present, mainstream RL algorithms are data-driven, which usually yield better asymptotic performance but much slower convergence compared with model-driven methods. This paper proposes mixed policy gradient (MPG) algorithm, which fuses the empirical data and the transition model in policy gradient (PG) to accelerate convergence without performance degradation. Formally, MPG is constructed as a weighted average of the data-driven and model-driven PGs, where the former is the derivative of the learned Q-value function, and the latter is that of the model-predictive return. To guide the weight design, we analyze and compare the upper bound of each PG error. Relying on that, a rule-based method is employed to heuristically adjust the weights. In particular, to get a better PG, the weight of the data-driven PG is designed to grow along the learning process while the other to decrease. Simulation results show that the MPG method achieves the best asymptotic performance and convergence speed compared with other baseline algorithms.

==> latex/appendices/addi_descs.tex <==
\section{Additional descriptions}\label{appendix.addi_desc}
% \subsection{General form of MPG}\label{appendix.general_mpg}
% The general form of the MPG is as follows,
% \begin{equation}
% \nonumber
% \nabla_{\theta}J^{\text{Mixed}} = \sum_{i\in \mathbb{I}}w_i \nabla_{\theta}J_i(\theta),
% \end{equation}
% where $\mathbb{I}$ is the set of used horizon lengths, $\mathbb{I} \subset \mathbb{N}$ and $0\in\mathbb{I}$, and $w_i (i\in\mathbb{I})$ are the weights to be determined. 
% % A corresponding heuristic weighting method is,
% % \begin{equation}
% % \nonumber
% % \begin{aligned}
% % w_i &= \frac{1/\text{Heur-Bias}_i}{\sum_k 1/\text{Heur-Bias}_k}, i\in \mathbb{I}\\
% % \text{Heur-Bias}_i &= \mathbb{E}_{s\sim \rho^{\pi_{\theta}}}\left\{ (R^{\text{True}}(s)-R^{\text{Mixed}}_i(s))^2 \right\}\\
% % R^{\text{True}}(s) &=\sum_{l=t}^{\infty} \gamma^{l-t} r_l \bigg|_{s_t=s}\\
% % R^{\text{Mixed}}_i(s) &=\sum_{l=t}^{i-1+t} \gamma^{l-t} \hat{r}_l + \gamma^{n} Q_{w, \hat{t+i}}\bigg|_{\hat{s}_t=s}.\\
% % \end{aligned}
% % \end{equation}
% A corresponding rule-based weighting method is
% \begin{equation}
% \nonumber
% \begin{aligned}
% w_i &= \mathrm{Softmax}(1/e_i), i\in\mathbb{I}\\
% e_i &=\left\{
% \begin{array}{ll}
%          \lambda^i, & \lambda\le1 \\
%          (2-\lambda)^{\max \mathbb{I}-i}, &\lambda>1\\
% \end{array} \right. ,\\
% \end{aligned}
% \end{equation}
% where $\lambda$ is a variable that linearly increases from $1-\eta$ to $1+\eta$ within iteration $T$ and remains $1+\eta$ thereafter, $\eta\in(0, 1)$ and $T$ are served as hyperparamters.

% \subsection{Basic description of the algorithms}\label{appendix.alg_desc}
% See Table \ref{tab.alg_desc}.
% \begin{table}[h]%[tbhp]
% \centering
% \caption{\MakeUppercase{Basic description of the algorithms.}}
% \label{tab.alg_desc}
% \begin{threeparttable}[h]
% \begin{tabular}{p{1.6cm}p{0.3cm}p{2.4cm}p{1.4cm}p{1cm}}
% \toprule
% Algorithm & D/S\tnote{*} & Value target & PG & Info source \\
% \midrule
% MPG-v1 & D & $n$-step TD & MPG & Data \& model \\
% MPG-v2 & D & Clipped double Q & MPG & Data \& model \\
% $n$-step DPG & D & $n$-step TD & DPG & Data \\
% $n$-step ADP & D & $n$-step TD & Model PG & Model \\
% TD3 & D & Clipped double Q & DPG & Data \\
% SAC & S & Clipped double Q & Soft PG & Data \\
% \bottomrule
% \end{tabular}
% \begin{tablenotes}
%      \item[*] Deterministic policy or Stochastic policy.
% \end{tablenotes}
% \end{threeparttable}
% \end{table}

% \subsection{Hyperparameters}\label{appendix.hyper}
% See Table \ref{table.hyper}.
% \begin{table}[!htp] 
% \centering
% \caption{\MakeUppercase{Detailed hyperparameters.}}
% \label{table.hyper}
% \begin{threeparttable}[h]
% \begin{tabular}{lc}
% \toprule
% Algorithm & Value \\
% \hline
% \emph{Shared} & \\
% \quad Optimizer &  Adam ($\beta_{1}=0.9, \beta_{2}=0.999$)\\
% \quad Approximation function  & MLP \\
% \quad Number of hidden layers & 2\\
% \quad Number of hidden units & 256\\
% \quad Nonlinearity of hidden layer& ELU\\
% % \quad Nonlinearity of output layer& linear\\
% \quad Replay buffer size & 5e5\\
% \quad Batch size & 256\\
% \quad Policy learning rate & Linear decay 3e-4 $\rightarrow$ 3e-6 \\
% \quad Value learning rate & Linear decay 8e-4 $\rightarrow$ 8e-6\\
% \quad Discount factor $\gamma$ & 0.98\\
% \quad Target smoothing coefficient $\tau$ & 0.005\\
% % \quad Reward scale & 0.01\\
% % \quad Update interval ($m$)& 2\\
% % \quad Target smoothing coefficient ($\tau$) & 0.001\\
% \quad Number of Actors &2\\
% \quad Number of Buffers &2\\
% \quad Number of Learners &12\\
% \hline
% \emph{MPG (v1, v2)} &\\ 
% % \quad Decay rate $\xi$ (for v1 only) &  0.01\\
% \quad Weighting schedule $\eta$, $T$ &  0.1, 9000/4000\tnote{*}\\
% \quad $H$ & 25\\
% \quad $n$ for value/policy learning & 25\\
% % \quad Update interval & 2 \\
% % \quad Exploration noise & $\epsilon\sim\mathcal{N}(0, 0.1)$\\
% \quad Number batch reuse & 10\\
% \quad Delayed update & 2\\
% \hline
% \emph{$n$-step DPG, $n$-step ADP} &\\ 
% \quad $n$ for value/policy learning & 25\\
% \quad Number batch reuse & 10\\
% \hline
% % \emph{$n$-step DPG} &\\ 
% % \quad Exploration noise & $\epsilon\sim\mathcal{N}(0, 0.1)$\\
% % \hline
% % \emph{TD3, SAC} &\\ 
% % \quad Number of Learners & 2\\
% % \quad Number batch reuse & 1\\
% % \hline
% \emph{TD3} &\\ 
% \quad Exploration noise & $\epsilon\sim\mathcal{N}(0, 0.1)$\\
% \quad Delayed update & 2\\
% \quad Policy smoothing noise & $\epsilon\sim\text{clip}(\mathcal{N}(0, 0.1), -0.5, 0.5)$\\
% \hline
% \emph{SAC} &\\ 
% \quad Fixed $\alpha$ & 0.03 \\
% \bottomrule
% \end{tabular}
% \begin{tablenotes}
%      \item[*] For path tracking and inverted pendulum tasks, respectively.
% \end{tablenotes}
% \end{threeparttable}
% \end{table}

==> latex/appendices/addi_results.tex <==
\section{Additional results}\label{appendix.addi_results}
Fig. \ref{fig.error} graphs the tracking errors of all baseline algorithms on the path tracking task. We calculate the tracking errors using the root mean squared over states of 5 episodes every 3000 iterations (each episode has a fixed length of 200). Specifically, the errors are calculated by
\begin{equation}
\nonumber
\text{Error}_{\dagger} = \sqrt{\mathbb{E}_{\dagger\in\mathbb{C}_{\dagger}}\left\{(\dagger - \dagger_{\text{ref}})^2\right\}}
\end{equation}
where $\text{Error}_{\dagger}, \dagger \in \{y, \phi, u\}$ is to denote the position error, heading angle error and velocity error, respectively. $\mathbb{C}_{\dagger}$ is the corresponding state collection of 5 episodes.
\begin{figure}[h]
\centering
\captionsetup[subfigure]{justification=centering}
\subfloat[Position error]{\label{fig.position_error}\includegraphics[width=0.4\textwidth]{Figures/path_tracking/addi/position_error.pdf}}\\
\subfloat[Heading angle error]{\label{fig.heading_angle_error}\includegraphics[width=0.4\textwidth]{Figures/path_tracking/addi/heading_angle_error.pdf}}\\
\subfloat[Velocity error]{\label{fig.velocity_error}\includegraphics[width=0.4\textwidth]{Figures/path_tracking/addi/velocity_error.pdf}}
\caption{Tracking errors of path tracking task. (a) Position error. (b) Heading angle error. (c) Velocity error. The solid lines correspond to the mean and the shaded regions correspond to 95\% confidence interval over 5 runs.}
\label{fig.error}
\end{figure}

\newpage
Besides, Fig. \ref{fig.cart_pole_error} graphs the state magnitudes on the inverted pendulum task, which is calculated by the root mean square over actions of 5 episodes every 3000 iterations. Specifically, the state magnitudes are calculated by
\begin{equation}
\nonumber
\text{State}_{\dagger} = \sqrt{\mathbb{E}_{\dagger\in\mathbb{C}_{\dagger}}\left\{\dagger^2\right\}}
\end{equation}
where $\text{State}_{\dagger}, \dagger \in \{x, \Dot{x}, \theta, \Dot{\theta}\}$ is to denote the magnitude of the cart position, cart velocity, pole angle and pole angular velocity, respectively. $\mathbb{C}_{\dagger}$ is the corresponding state collection of 5 episodes.

\newpage
\quad
\begin{figure}[!htbp]
\centering
\captionsetup[subfigure]{justification=centering}
\subfloat[Cart position]{\label{fig.cart_position}\includegraphics[width=0.4\textwidth]{Figures/inverted_pendulum/addi/cart_position.pdf}}\\
\subfloat[Cart velocity]{\label{fig.cart_velocity}\includegraphics[width=0.4\textwidth]{Figures/inverted_pendulum/addi/cart_velocity.pdf}}\\
\subfloat[Pole angle]{\label{fig.pole_angle}\includegraphics[width=0.4\textwidth]{Figures/inverted_pendulum/addi/pole_angle.pdf}}\\
\subfloat[Pole angular velocity]{\label{fig.pole_angular_velocity}\includegraphics[width=0.4\textwidth]{Figures/inverted_pendulum/addi/pole_angular_velocity.pdf}}
\caption{State magnitudes of inverted pendulum task. (a) Cart position. (b) Cart velocity. (c) Pole angle. (d) Pole angular velocity. The solid lines correspond to the mean and the shaded regions correspond to 95\% confidence interval over 5 runs.}
\label{fig.cart_pole_error}
\end{figure}




==> latex/appendices/baseline_algos.tex <==
% \section{Baseline algorithms}\label{appendix.baseline_algs}
% \subsection{$n$-step DPG}\label{appendix.ndpg}
% Suppose the action-value function and policy are approximated by parameterized functions $Q_w(s, a)$ and $\pi_{\theta}(s)$ respectively. Given separate target action-value function $Q_{w'}$ and policy $\pi_{\theta'}$, the update target of $Q_{w}$ is calculated the same as MPG:
% \begin{equation}
% \nonumber
% R^{\text{Target}}(s, a) = \sum_{l=t}^{t+n-1} \gamma^{l-t} r_l + \gamma^{n} Q_{w'}(s_{t+n}, \pi_{\theta'}(s_{t+n})) \bigg|_{s_t=s, a_t=a}.
% \end{equation}
% where $s_{t+i} \sim p(\cdot|s_{t+i-1}, \pi_{\theta}(s_{t+i-1})), i \ge 1$;
% $r_{t+i} := r(s_{t+i}, \pi_{\theta}(s_{t+i})), i \ge 0$. The action-value function can be trained by directly minimizing
% \begin{equation}
% \nonumber
% J_Q(w) = \mathbb{E}_{s,a\sim \mathcal{B}}\left\{\frac{1}{2}(R^{\text{Target}}(s, a) - Q_w(s,a))^2\right\}.
% \end{equation}
% The policy can be learned by directly maximizing the learned action-value function, same as DPG:
% \begin{equation}
% \nonumber
% J_{\pi}(\theta) = \mathbb{E}_{s\sim \mathcal{B}}\left\{Q_w(s, \pi_{\theta}(s))\right\}.
% \end{equation}
% The pseudo-code of $n$-step DPG is shown in Algorithm \ref{alg.ndpg}.

% \begin{algorithm}[htbp]
%   \caption{$n$-step DPG}
%   \label{alg.ndpg}
% \begin{algorithmic}
%   \STATE {\bfseries Initialize:} critic network $Q_w$ and actor network $\pi_{\theta}$ with random parameters $w$, $\theta$, target parameters $w' \leftarrow w, \theta' \leftarrow \theta$, batch size $N$, initial buffer $\mathcal{B}$ with $N$ samples, exploration noise $\epsilon$, target smoothing coefficient $\tau$, learning rate $\beta_w, \beta_{\theta}$
%   \FOR{each iteration $k$}
%       \STATE Collect a batch of transitions using $\pi_{\theta}$ with noise $\epsilon$, store in $\mathcal{B}$
%       \STATE Sample $N$ transitions $\{s_i, a_i, r_i, s_{i+1}\}_{i=0:N-1}$ from $\mathcal{B}$
%       \STATE Update value $w \leftarrow w - \beta_w \nabla_{w}J_Q(w)$
%       \STATE Update policy $\theta \leftarrow \theta + \beta_{\theta} \nabla_{\theta}J_{\pi}(\theta)$
%       \STATE Update target networks:
%       \STATE \quad $w' \leftarrow \tau w + (1-\tau) w'$
%       \STATE \quad \ $\theta' \leftarrow \tau \theta + (1-\tau) \theta'$
%   \ENDFOR
% \end{algorithmic}
% \end{algorithm}

% \subsection{$n$-step ADP}\label{appendix.nadp}
% Suppose the action-value function and policy are approximated by parameterized functions $Q_w(s, a)$ and $\pi_{\theta}(s)$ respectively. Given separate target action-value function $Q_{w'}$ and policy $\pi_{\theta'}$, the update target of $Q_{w}$ is calculated as follows:
% \begin{equation}
% \nonumber
% R^{\text{Target}}(s, a) = \sum_{l=t}^{t+n-1} \gamma^{l-t} \hat{r}_l + \gamma^{n} Q_{w'}(\hat{s}_{t+n}, \pi_{\theta'}(\hat{s}_{t+n})) \bigg|_{\hat{s}_t=s, \hat{a}_t=a}.
% \end{equation}
% The action-value function can be trained by directly minimizing
% \begin{equation}
% \nonumber
% J_Q(w) = \mathbb{E}_{s,a\sim \mathcal{B}}\left\{\frac{1}{2}(R^{\text{Target}}(s, a) - Q_w(s,a))^2\right\}.
% \end{equation}
% The policy can be learned by directly maximizing $n$-step model return:
% \begin{equation}
% \nonumber
% J_{\pi}(\theta) = \mathbb{E}_{s\sim \mathcal{B}}\left\{\mathbb{E}_{\substack{\hat{s}_{t+1},\\ \dots, \\\hat{s}_{t+n}}}\left\{\sum_{l=t}^{n-1+t} \gamma^{l-t} \hat{r}_l + \gamma^{n} Q_{w, \hat{t+n}} \right\}\bigg|\hat{s}_t=s\right\}.
% \end{equation}
% where $\hat{s}_{t+i} \sim f(\cdot|\hat{s}_{t+i-1}, \pi_{\theta}(\hat{s}_{t+i-1})), i \ge 1$;
% $\hat{r}_{t+i} := r(\hat{s}_{t+i}, \pi_{\theta}(\hat{s}_{t+i})), i \ge 0$;  $Q_{w,\hat{t+i}}:=Q_w(\hat{s}_{t+i},\pi_{\theta}(\hat{s}_{t+i})), i \ge 1$. The pseudo-code of $n$-step ADP is shown in Algorithm \ref{alg.nadp}.

% \begin{algorithm}[htbp]
%   \caption{$n$-step ADP}
%   \label{alg.nadp}
% \begin{algorithmic}
%   \STATE {\bfseries Initialize:} critic network $Q_w$ and actor network $\pi_{\theta}$ with random parameters $w$, $\theta$, target parameters $w' \leftarrow w, \theta' \leftarrow \theta$, batch size $N$, initial buffer $\mathcal{B}$ with $N$ samples, target smoothing coefficient $\tau$, learning rate $\beta_w, \beta_{\theta}$
%   \FOR{each iteration $k$}
%       \STATE Collect a batch of transitions using $\pi_{\theta}$, store in $\mathcal{B}$
%       \STATE Sample $N$ transitions $\{s_i, a_i, r_i, s_{i+1}\}_{i=0:N-1}$ from $\mathcal{B}$
%       \STATE Update value $w \leftarrow w - \beta_w \nabla_{w}J_Q(w)$
%       \STATE Update policy $\theta \leftarrow \theta + \beta_{\theta} \nabla_{\theta}J_{\pi}(\theta)$
%       \STATE Update target networks:
%       \STATE \quad $w' \leftarrow \tau w + (1-\tau) w'$
%       \STATE \quad \ $\theta' \leftarrow \tau \theta + (1-\tau) \theta'$
%   \ENDFOR
% \end{algorithmic}
% \end{algorithm}

==> latex/defs.tex <==
\newcommand{\cmt}[1]{{\footnotesize\textcolor{red}{#1}}}
\newcommand{\lcmt}[1]{{\footnotesize\textcolor{red}{#1}}\\}
\newcommand{\todo}[1]{\cmt{(TODO: #1)}}

% 可主要定义【常用】的符号，以简化上下标、空格、左右括号等
% 以下定义的符号不用加括号，如果直接作为上下标，在正文加就好，如果不作为上下标，可能有在其上添加上下标的需求，这个时候如果加了括号，就很麻烦
\newcommand{\lb}[1]{\left [ #1 \right.}
\newcommand{\rb}[1]{\left. #1 \right ]}
\newcommand{\lrb}[1]{\left [ #1 \right ]}
\newcommand{\lp}[1]{\left ( #1 \right.}
\newcommand{\rp}[1]{\left. #1 \right )}
\newcommand{\lrp}[1]{\left ( #1 \right )}

\newcommand{\lc}[1]{\left \{ #1 \right.}
\newcommand{\rc}[1]{\left. #1 \right \}}
\newcommand{\lrc}[1]{\left \{ #1 \right \}}

\renewcommand{\lVert}[1]{\left \Vert #1 \right.}
\renewcommand{\rVert}[1]{\left. #1 \right \Vert}
\newcommand{\lrVert}[1]{\left \Vert #1 \right \Vert}

\renewcommand{\lvert}[1]{\left \vert #1 \right.}
\renewcommand{\rvert}[1]{\left. #1 \right \vert}
\newcommand{\lrvert}[1]{\left \vert #1 \right \vert}

\newcommand{\lrangle}[1]{\left \langle #1 \right \rangle}

% Math operators and functions
\newcommand{\E}[2]{\operatorname{\symbb{E}}_{#1} \lrb{#2}}
\newcommand{\D}[1]{\operatorname{\symbb{D}}\lrb{#1}}
% \newcommand{\Eleft}[2]{\operatorname{\symbb{E}}_{#1}\lb#2\right.}
% \newcommand{\Eright}[1]{\left.#1\rb}
\newcommand{\Ed}[2]{\operatorname*{\symbb{E}}_{#1} \lrb{#2}}
\newcommand{\Eleftd}[2]{\operatorname*{\symbb{E}}_{#1}\lb{#2}}
\newcommand{\Erightd}[1]{\rb{#1}}
\newcommand{\EEE}{\symbb{E}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\Max}{max}
\DeclareMathOperator*{\Min}{min}

% Other helpers
\newcommand{\voidarg}{{\,\cdot\,}}

% IDC
\newcommand{\xspace}{\symcal{X}}
\newcommand{\xspaceobst}{\symcal{X}_{\text{obst}}}
\newcommand{\x}{\symbf{x}}
\newcommand{\y}{\symbf{y}}
\newcommand{\xego}{\x_{\text{ego}}}
\newcommand{\xref}{\x_{\text{ref}}}
\newcommand{\xroad}{\x_{\text{road}}}
\newcommand{\xlight}{\x_{\text{light}}}
\newcommand{\xobst}{\x_{\text{obst}}}
\newcommand{\xobstj}{\x^j_{\text{obst}}}
\newcommand{\xobstone}{\x^1_{\text{obst}}}
\newcommand{\xobstN}{\x^N_{\text{obst}}}
\newcommand{\xobstM}{\x^M_{\text{obst}}}
\newcommand{\xset}{\x_{\text{set}}}
\newcommand{\xelse}{\x_{\text{else}}}
\newcommand{\uspace}{\symcal{U}}
\newcommand{\uaction}{\symbf{u}}
\newcommand{\uopt}{\symbf{u}\opt}
\newcommand{\ut}{\symbf{u}^t}
\newcommand{\utp}{\symbf{u}^{t+1}}
\newcommand{\tauref}{\tau_{\text{ref}}}
\newcommand{\taurefk}{\tauref^k}
\newcommand{\taurefopt}{\tau^*_{\text{ref}}}
\newcommand{\stateset}{\Pi_{\text{state}}}
\newcommand{\stateseti}{\stateset^i}
\newcommand{\statesetk}{\stateset^k}
\newcommand{\taurefset}{\Pi_{\text{ref}}}
\newcommand{\safepolicyset}{\Pi_{\text{safe}}}

\newcommand{\Jpolicy}{J_{\policy}}
\newcommand{\Jcpolicy}{J^c_{\policy}}
\newcommand{\JQ}{J_Q}
\newcommand{\pf}{\sigma}
\newcommand{\Prob}{\symcal{P}}

\newcommand{\tauhat}{\hat{\tau}}

\newcommand{\acccmd}{\Alpha}
\newcommand{\steercmd}{\Theta}



%obj：要优化的变量全在括号里面，J的上下标可以标识说明性符号，或编号，也可以不标上下标

% text
\newcommand{\obst}{\text{obst}}
\newcommand{\ego}{\text{ego}}
\newcommand{\navi}{\text{navi}}
\newcommand{\lane}{\text{lane}}
\newcommand{\rref}{\text{ref}}
\newcommand{\curve}{\text{curve}}
\renewcommand{\rule}{\text{rule}}
\newcommand{\map}{\text{map}}
\newcommand{\light}{\text{light}}
\newcommand{\road}{\text{road}}
\newcommand{\DOFWE}{\text{DOFWE}}
\newcommand{\lbd}{\text{lb}}
\newcommand{\hbd}{\text{hb}}
\newcommand{\safe}{\text{safe}}
\newcommand{\vio}{\text{vio}}
\newcommand{\pred}{\text{pred}}
\newcommand{\data}{\text{data}}
\newcommand{\model}{\text{model}}
\newcommand{\mixed}{\text{mixed}}
\newcommand{\old}{\text{old}}
\newcommand{\mpc}{\text{mpc}}
\newcommand{\track}{\text{track}}
\newcommand{\energy}{\text{energy}}
\newcommand{\stability}{\text{stability}}
\newcommand{\smooth}{\text{smooth}}
\renewcommand{\stop}{\text{stop}}

% MDP
\newcommand{\sspace}{\symcal{S}}
\newcommand{\aspace}{\symcal{A}}
\newcommand{\state}{\symbf{s}}
\newcommand{\statenoise}{\symbf{\epsilon}}
\newcommand{\sprime}{\symbf{s}^{\prime}}
\newcommand{\stm}{\state_{t-1}}
\renewcommand{\st}{\state_t}
% \renewcommand{\sl}{\state_l}
% \newcommand{\slp}{\state_{l+1}}
\newcommand{\stp}{\state_{t+1}}
\newcommand{\stpi}{\state_{t+i}}
\newcommand{\stpn}{\state_{t+n}}
\newcommand{\si}{\state_i}
\newcommand{\simm}{\state_{i-1}}
\newcommand{\sip}{\state_{i+1}}
\newcommand{\sipn}{\state_{i+n}}

\newcommand{\action}{\symbf{a}}
\newcommand{\aprime}{\symbf{a}^{\prime}}
\newcommand{\atm}{\action_{t-1}}
\newcommand{\at}{\action_t}
% \newcommand{\al}{\action_l}
\newcommand{\atp}{\action_{t+1}}
\newcommand{\atpi}{\action_{t+i}}
\newcommand{\atpn}{\action_{t+n}}
\newcommand{\ai}{\action_i}
\newcommand{\aip}{\action_{i+1}}
\newcommand{\aipn}{\action_{i+n}}
\newcommand{\opt}{^*}
\newcommand{\obs}{\symbf{o}}
\newcommand{\otm}{\obs_{t-1}}
\newcommand{\ot}{\obs_t}
% \newcommand{\ol}{\obs_l}
\newcommand{\oi}{\obs_i}
\newcommand{\oprime}{\obs^{\prime}}
\newcommand{\otp}{\obs_{t+1}}
\newcommand{\otpn}{\obs_{t+n}}

% Model correspondence for MDP
\newcommand{\statehat}{\hat{\state}}
\newcommand{\stmhat}{\statehat_{t-1}}
\newcommand{\sthat}{\statehat_t}
% \newcommand{\slhat}{\statehat_l}
\newcommand{\sihat}{\statehat_i}
\newcommand{\stphat}{\statehat_{t+1}}
\newcommand{\stpihat}{\statehat_{t+i}}
\newcommand{\slphat}{\statehat_{l+1}}
\newcommand{\siphat}{\statehat_{i+1}}
\newcommand{\stpnhat}{\statehat_{t+n}}

\newcommand{\actionhat}{\hat{\action}}
\newcommand{\atmhat}{\actionhat_{t-1}}
\newcommand{\athat}{\actionhat_t}
% \newcommand{\alhat}{\actionhat_l}
\newcommand{\aihat}{\actionhat_i}
\newcommand{\atphat}{\actionhat_{t+1}}
\newcommand{\atpihat}{\actionhat_{t+i}}
\newcommand{\atpnhat}{\actionhat_{t+n}}

% Rewards and costs
\newcommand{\reward}{r}
\newcommand{\rtm}{\reward_{t-1}}
\newcommand{\rt}{\reward_t}
% \newcommand{\rl}{\reward_l}
\newcommand{\ri}{\reward_i}
\newcommand{\rtp}{\reward_{t+1}}
\newcommand{\rtpi}{\reward_{t+i}}
\newcommand{\rtpn}{\reward_{t+n}}

\newcommand{\cost}{c}
\newcommand{\ctm}{\cost_{t-1}}
\newcommand{\ct}{\cost_t}
% \newcommand{\cl}{\cost_l}
\newcommand{\ci}{\cost_i}
\newcommand{\ctp}{\cost_{t+1}}
\newcommand{\ctpi}{\cost_{t+i}}
\newcommand{\ctpn}{\cost_{t+n}}

% Model correspondence for Rewards and costs
\newcommand{\rewardhat}{\hat{r}}
\newcommand{\rtmhat}{\rewardhat_{t-1}} 
\newcommand{\rthat}{\rewardhat_t}
% \newcommand{\rlhat}{\rewardhat_l}
\newcommand{\rihat}{\rewardhat_i}
\newcommand{\rtphat}{\rewardhat_{t+1}}
\newcommand{\rtpihat}{\rewardhat_{t+i}}
\newcommand{\rtpnhat}{\rewardhat_{t+n}}

\newcommand{\costhat}{\hat{c}}
\newcommand{\ctmhat}{\costhat_{t-1}}
\newcommand{\cthat}{\costhat_t}
\newcommand{\clhat}{\costhat_l}
\newcommand{\cihat}{\costhat_i}
\newcommand{\ctphat}{\costhat_{t+1}}
\newcommand{\ctpihat}{\costhat_{t+i}}
\newcommand{\ctpnhat}{\costhat_{t+n}}

% V function
\newcommand{\vpolicy}{v^{\policy}}
\newcommand{\vpolicywithparams}{v^{\policywithparams}}
\newcommand{\Vwithparams}{V_{\vparams}}

\newcommand{\vdiamond}{v_{\diamond}}
\newcommand{\vdiamondopt}{\vdiamond\opt}
\newcommand{\vdiamondpolicy}{\vdiamond^{\policy}}
\newcommand{\vdiamondpolicywithparams}{\vdiamond^{\policywithparams}}
\newcommand{\Vdiamond}{V_{\diamond}}
\newcommand{\Vwithdiamondparams}{V_{\vdiamondparams}}

\newcommand{\vr}{v_r}
\newcommand{\vropt}{\vr\opt}
\newcommand{\vrpolicy}{\vr^{\policy}}
\newcommand{\vrpolicywithparams}{\vr^{\policywithparams}}
\newcommand{\Vr}{V_r}
\newcommand{\Vwithrparams}{V_{\vrparams}}

\newcommand{\vc}{v_c}
\newcommand{\vcopt}{\vc\opt}
\newcommand{\vcpolicy}{\vc^{\policy}}
\newcommand{\vcpolicywithparams}{\vc^{\policywithparams}}
\newcommand{\Vc}{V_c}
\newcommand{\Vwithcparams}{V_{\vcparams}}

% Q function
\newcommand{\qpolicy}{q^{\policy}}
\newcommand{\qpolicywithparams}{q^{\policywithparams}}
\newcommand{\Qwithparams}{Q_{\qparams}}

\newcommand{\qdiamond}{q_{\diamond}}
\newcommand{\qdiamondopt}{\qdiamond^*}
\newcommand{\qdiamondpolicy}{q^{\policy}_{\diamond}}
\newcommand{\Qdiamond}{Q_{\diamond}}
\newcommand{\Qwithdiamondparams}{Q_{\qdiamondparams}}

\newcommand{\qr}{q_r}
\newcommand{\qropt}{\qr^*}
\newcommand{\qrpolicy}{q^{\policy}_r}
\newcommand{\qrpolicywithparams}{q^{\policywithparams}_r}

\newcommand{\Qr}{Q_r}
\newcommand{\Qwithrparams}{Q_{\qrparams}}
\newcommand{\Qwithrparamsopt}{Q_{\qrparamsopt}}

\newcommand{\qc}{q_c}
\newcommand{\qcopt}{\qc\opt}
\newcommand{\qcpolicy}{q^{\policy}_c}
\newcommand{\qcpolicywithparams}{q^{\policywithparams}_c}
\newcommand{\Qc}{Q_c}
\newcommand{\Qwithcparams}{Q_{\qcparams}}
\newcommand{\Qwithcparamsopt}{Q_{\qcparamsopt}}

% Policy and params
\newcommand{\policy}{\pi}
\newcommand{\policyopt}{\policy^*}
\newcommand{\policycirc}{\policy^{\circ}}
\newcommand{\policywithparams}{\policy_{\pparams}}
\newcommand{\policywithparamsopt}{\policy_{\pparamsopt}}
\newcommand{\pparams}{\symbf{\theta}}
\newcommand{\pparamsopt}{\pparams\opt}

\newcommand{\qparams}{\symbf{\omega}}
\newcommand{\qparamsopt}{\qparams\opt}
\newcommand{\qdiamondparams}{\qparams_{\diamond}}
\newcommand{\qrparams}{\qparams_r}
\newcommand{\qcparams}{\qparams_c}
\newcommand{\qrparamsopt}{\qparams\opt_r}
\newcommand{\qcparamsopt}{\qparams\opt_c}
\newcommand{\qrparamspolicywithparams}{\qparams_r^{\policywithparams}}
\newcommand{\qcparamspolicywithparams}{\qparams_c^{\policywithparams}}


% \newcommand{\qoneparams}{{\omega^1}}
% \newcommand{\qtwoparams}{{\omega^1}}
% \newcommand{\qonerparams}{{\omega^1_r}}
% \newcommand{\qtworparams}{{\omega^2_r}}
% \newcommand{\qonecparams}{{\omega^1_c}}
% \newcommand{\qtwocparams}{{\omega^2_c}}

\newcommand{\vparams}{\symbf{\omega}}
\newcommand{\vdiamondparams}{\vparams_{\diamond}}
\newcommand{\vrparams}{\vparams_r}
\newcommand{\vcparams}{\vparams_c}

\newcommand{\ptargetparams}{\bar{\pparams}}

\newcommand{\qtargetparams}{\bar{\qparams}}
\newcommand{\qrtargetparams}{\bar{\qrparams}}
\newcommand{\qctargetparams}{\bar{\qcparams}}

% \newcommand{\qonetargetparams}{{\bar\qoneparams}}
% \newcommand{\qtwotargetparams}{{\bar\qtwoparams}}
% \newcommand{\qonertargetparams}{{\bar\qonerparams}}
% \newcommand{\qtwortargetparams}{{\bar\qtworparams}}
% \newcommand{\qonectargetparams}{{\bar\qonecparams}}
% \newcommand{\qtwoctargetparams}{{\bar\qtwocparams}}

\newcommand{\vtargetparams}{\bar{\vparams}}
\newcommand{\vrtargetparams}{\bar{\vrparams}}
\newcommand{\vctargetparams}{\bar{\vcparams}}

\newcommand{\Qhatwtpn}{\hat{Q}_{\qparams,t+n}}
\newcommand{\Qhatwtp}{\hat{Q}_{\qparams,t+1}}
\newcommand{\Qhatwt}{\hat{Q}_{\qparams,t}}
\newcommand{\Qhatwtpi}{\hat{Q}_{\qparams,t+i}}

% encoding params
\newcommand{\eparams}{\symbf{\psi}}


% Distributions.
\newcommand{\gauss}{\symcal{N}}
\newcommand{\buffer}{\symcal{B}}
\newcommand{\ifelse}{\symbb{I}}
\newcommand{\targetnetsyncrate}{\iota}


% Other.
\newcommand{\inv}{^{-1}}
\newcommand{\T}{^{\top}}
\newcommand{\reals}{\symbb{R}}
\newcommand{\discount}{\gamma}
\newcommand{\Exp}{\mathop{\mathbb E}\displaylimits}
\newcommand{\dvf}{\rho^{\policy}(\state)}
\newcommand{\dvfwithparams}{\rho^{\policywithparams}(\state)}

\newcommand{\VNE}{\text{V}_{\text{NE}}}
\newcommand{\VNS}{\text{V}_{\text{NS}}}
\newcommand{\VNW}{\text{V}_{\text{NW}}}
\newcommand{\VES}{\text{V}_{\text{ES}}}
\newcommand{\VEW}{\text{V}_{\text{EW}}}
\newcommand{\VEN}{\text{V}_{\text{EN}}}
\newcommand{\VSW}{\text{V}_{\text{SW}}}
\newcommand{\VSN}{\text{V}_{\text{SN}}}
\newcommand{\VSE}{\text{V}_{\text{SE}}}
\newcommand{\VWN}{\text{V}_{\text{WN}}}
\newcommand{\VWE}{\text{V}_{\text{WE}}}
\newcommand{\VWS}{\text{V}_{\text{WS}}}

\newcommand{\BNS}{\text{B}_{\text{NS}}}
\newcommand{\BEW}{\text{B}_{\text{EW}}}
\newcommand{\BSN}{\text{B}_{\text{SN}}}
\newcommand{\BWE}{\text{B}_{\text{WE}}}

\newcommand{\PNW}{\text{P}_{\text{NW}}}
\newcommand{\PNE}{\text{P}_{\text{NE}}}
\newcommand{\PEN}{\text{P}_{\text{EN}}}
\newcommand{\PES}{\text{P}_{\text{ES}}}
\newcommand{\PSE}{\text{P}_{\text{SE}}}
\newcommand{\PSW}{\text{P}_{\text{SW}}}
\newcommand{\PWS}{\text{P}_{\text{WS}}}
\newcommand{\PWN}{\text{P}_{\text{WN}}}

